TaxoLLaMA: WordNet-based Model for Solving Multiple Lexical Semantic Tasks

In this paper, we explore the capabilities of LLMs in capturing lexical-semantic knowledge from WordNet on the example of the LLaMA-2-7b model and test it on multiple lexical semantic tasks. As the outcome of our experiments, we present TaxoLLaMA, the everything-in-one model, lightweight due to 4-bit quantization and LoRA. It achieves 11 SotA results, 4 top-2 results out of 16 tasks for the Taxonomy Enrichment, Hypernym Discovery, Taxonomy Construction, and Lexical Entailment tasks. Moreover, it demonstrates very strong zero-shot performance on Lexical Entailment and Taxonomy Construction with no fine-tuning. We also explore its hidden multilingual and domain adaptation capabilities with a little tuning or few-shot learning. All datasets, code, and model are available online at https://github.com/VityaVitalich/TaxoLLaMA

==> tables/enrich.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
 & MAG-CS & MAG-PSY & Noun & Verb \\ 
\midrule
GenTaxo & 23.9 & 46.4 & 28.6 & 42.8 \\
TMN & 24.3 & 53.1 & 36.7 & 35.4 \\
TaxoExpan & 19.3 & 44.1 & 39.0 & 32.5 \\
TaxoEnrich & 57.8 & 58.3 & 44.2 & 45.2 \\
\midrule
UniTax zero-shot & 7.4 & 7.3 & - & - \\
UniTax-b zero-shot & 8.5 & 6.6 & - & - \\
\midrule
UniTax & 24.9 & 29.8 & 48.0 & 52.4 \\
UniTax-b & 30.2 & 31.4 & 45.9 & 51.9 \\
UniTax ranker & 34.8 & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Revised MRR Performance Across Tasks for Taxonomy Enrichment}
\label{table:revised_mrr_performance}
\end{table}

==> tables/entailment.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cc}
\toprule
 & Roc Auc & AP \\ 
\midrule
UniTax bench & 52.82 & 54.24 \\
UniTax & 50.89 & 51.61 \\
UniTax verb & 69.28 & 69.51 \\
SOTA & 75.86 & 67.47 \\
SOTA without tricks & 65.44 & 65.66 \\
\bottomrule
\end{tabular}
}
\caption{Performance on lexical entailment ANT dataset}
\label{table:performance_metrics}
\end{table}

==> tables/hypernym_prediction.tex <==
% \begin{table}[h]
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{l|ccccc}
% \toprule
%       & 1A    & 1B    & 1C    & 2A    & 2B    \\ 
% \midrule
% SemEval best      &  36.10     & 25.14 & 37.56 &   54.64   & 60.93     \\ 
% Prev work & 45.22 & - & - & - & - \\
% HyperBox & - & - & - & 27.79 & 41.39 \\
% RMM & 39.07 & - & - & 54.89 & 74.75 \\
% Hybrid &  34.07 & - & - &  64.47 & 77.24 \\
% \midrule
% UniTax         & 54.39 & 51.58 & 57.44 & 77.32 & 80.6  \\
% UniTax zero-shot     & 38.05 & 1.95  & 2.21  & 43.09 & 42.7  \\
% UniTax bench    & 51.59 & 50.95 & 58.61 & 73.82 & 78.63 \\
% UniTax bench zero-shot & 37.66 & 1.47  & 2.08  & 42.2  & 44.36 \\
% \bottomrule
% \end{tabular}
% }
% \caption{MRR performance on Hypernym Discovery Task}
% \label{table:hd_all}
% \end{table}

\begin{table}[h!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
      & 1A    & 2A    & 2B    \\ 
\midrule
SemEval best      &  36.10     &  54.64   & 60.93     \\ 
Prev work & 45.22 & - & - \\
RMM & 39.07 & 54.89 & 74.75 \\
Hybrid &  34.07 &  64.47 & 77.24 \\
\midrule
UniTax zero-shot     & 38.05 & 43.09 & 42.7  \\
UniTax-b zero-shot & 37.66 & 42.2  & 44.36 \\
\midrule
UniTax         & 54.39 & 77.32 & 80.6  \\
UniTax-b    & 51.59 & 73.82 & 78.63 \\
\bottomrule
\end{tabular}
}
\caption{MRR performance on Hypernym Discovery Task}
\label{table:hd_english}
\end{table}

\begin{table}[h]
\centering
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{l|cc}
\toprule
      & 1B    & 1C    \\ 
\midrule
300-sparsans r1       & 25.14 & 37.56 \\ 
NLP HZ & 19.19 & 28.27 \\
\midrule
UniTax zero-shot     & 1.95  & 2.21  \\
UniTax-b zero-shot & 1.47  & 2.08  \\
\midrule
UniTax         & 51.58 & 57.44 \\
UniTax-b    & 50.95 & 58.61 \\
\bottomrule
\end{tabular}
}
\caption{MRR performance on Hypernym Discovery Task}
\label{table:hd_language}
\end{table}

==> tables/texeval.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}
{
\begin{tabular}{l|ccc}
\toprule
 & Sci & Env & Food \\ 
\midrule
TexEval-2 best  & 31.3 & 30.0 &  36.01 \\
Graph2Taxo pure & 39.0 & 37.0 &  - \\
Graph2Taxo best & 47.0 & 40.0 &  - \\
LMScorer best & 31.8 & 26.4 & 24.9 \\
RestrictMLM & 37.9 & 23.0 & 24.9 \\
TAXI+ & 41.4 & 30.9 & 34.1 \\
\midrule
UniTax & 44.55 & 45.13 & 51.71 \\
UniTax bench & 42.36 & 44.82 & 51.18 \\
\bottomrule
\end{tabular}
}
\caption{F1 score for TExEval}
\label{table:new_values}
\end{table}
